The Security War in File Systems: An Empirical Study from A Vulnerability-Centric Perspective

This paper presents a systematic study on the security of modern file systems, following a vulnerability-centric perspective. Specifically, we collected 377 file system vulnerabilities committed to the CVE database in the past 20 years. We characterize them from four dimensions that include why the vulnerabilities appear, how the vulnerabilities can be exploited, what consequences can arise, and how the vulnerabilities are fixed. This way, we build a deep understanding of the attack surfaces faced by file systems, the threats imposed by the attack surfaces, and the good and bad practices in mitigating the attacks in file systems. We envision that our study will bring insights towards the future development of file systems, the enhancement of file system security, and the relevant vulnerability mitigating solutions.

==> Tables/cve-components.tex <==
\begin{table}[t]
    \footnotesize
        \caption{The major vulnerable \textit{fs} components in Linux.}
        \vspace{-2ex}
    \label{tab:domain}
    \centering
	\begin{tabular}{|m{70pt}<{\raggedleft}|p{40pt}<{\raggedright}|}
                \hline
		\textbf{FS Component} & \textbf{Percentage}  \\
        \hline
		Index management                    & 39\% \\  
		Block management & 21\%\\
		%Permission model                     & 14\% 
		Page Cache & 12\%\\
        \hline
        %\textbf{Total} & \multicolumn{3}{r}{157}\\
       % \hline
    \end{tabular}
        \vspace{-4ex}
\end{table}

==> component.tex <==

%\begin{table}[!tph]
%    \footnotesize
%        \caption{The most vulnerable \textit{fs} components in Linux.}
%        \vspace{-2ex}
%    \label{tab:domain}
%    \centering
%    \begin{tabular}{m{70pt}<{\raggedleft}|p{85pt}<{\raggedright}}
%                \hline
%                \textbf{Name} & \textbf{\% of studied CVEs}  \\
%        \hline
%        Inode management                    & 39\% \\
%        Block management           & 21\% \\
%        Permission model                     & 14\% \\
%        Page cache                    & 12\% \\
%        \hline
%        %\textbf{Total} & \multicolumn{3}{r}{157}\\
%       % \hline
%    \end{tabular}
%        \vspace{-3ex}
%\end{table}

\subsection{Approaches to Exploit FS Vulnerabilities}
%In this section, we present the common approaches used by adversaries to exploit \textit{fs} vulnerabilites. 
%According to our study, 
We identify that adversaries use three common approaches to exploit \textit{fs} 
vulnerabilities: \textit{fs} components, features, and bugs. 

\subsubsection{Exploiting Vulnerable FS Components}
\label{sec:dimension2}
%\subsection{Overview}
%The virtual file system (VFS) in Linux kernel specifies a set of interfaces and data structures for 
%the underlying file system implementations. As a result, Linux file systems share similar system 
%design and structures, such as inode, superblock. On the other side, different file systems also have 
%their unique features. For example, file systems have diversified crash-safety model, e.g., journaling, 
%shadow paging, log-structuring. 
%After studying the generic consequences and causes of \textit{fs} vulnerabilities, 
We now discuss how adversaries can exploit vulnerable \textit{fs} components to launch their attacks. 
We list the most vulnerable \textit{fs} components in Table~\ref{tab:domain}. 
%according to our study 
%on the vulnerability distribution in file systems. 
%We will discuss these vulnerable \textit{fs} components respectively. 




%\begin{table}[t]
%    \footnotesize
%        \caption{The most vulnerable \textit{fs} components in Linux.}
%        \vspace{-3ex}
%    \label{tab:domain}
%    \centering
%    \begin{tabular}{m{100pt}<{\raggedleft}|p{25pt}<{\raggedright}}
%                \hline
%                \textbf{Name} & \textbf{\#CVEs}  \\
%        \hline
%        Inode management                    & 43 \\
%        Permission model                     & 22 \\
%        %Namespace management                & 16 \\
%        Page cache                    & 13 \\
%        Block allocation           & 13 \\
%        Superblock management          & 12 \\
%%        File management                    & 11 \\
%%        Crash-safety model                    & 7 \\
%        Dentry management           & 6 \\
%        \hline
%        %\textbf{Total} & \multicolumn{3}{r}{157}\\
%       % \hline
%    \end{tabular}
%    %    \vspace{-3ex}
%\end{table}


%\textbf{Inode Management (39\%).}
\noindent
\textbf{\texttt{F09:} Index management is the most vulnerable component (39\%).}
Our study shows that the core \textit{fs} component--inode management--is the most vulnerable part 
in \textit{fs}. %in which the extended attribute management is the most vulnerable part. 
This is probably due to its complexity of the extended attribute management.
%Extended attribute management of file systems is flexible and complicated. 
For example, Ext4 supports three on-disk formats to store extended attributes, including 
inside \emph{inode}, additional block, and dedicated \emph{inode}. 
When the size of file extended attribute is small, 
Ext4 stores the extended attributes inside the \emph{inode} by default. When the attribute size 
is large, Ext4 will use an additional block to store the extended attributes. 
We find that a majority of the vulnerabilities are exploited through corrupted images after adjusting 
the storage format of these extended attributes 
(e.g., \texttt{CVE-2018-11412}). 
%\jian{Need more inspiring insights about index management, we need to discuss more about why inode 
%is the most vulnerable component, how should we redesign inode in the future}
%Similar issues will happen in the inline data management, 
%adversaries would exploit these vulnerabilities to crash the file systems. 

%Ext4 stores the inline data in the \textit{i\_data} field in the inode when the size is small than 
%60 bytes. When the size of inline data covert to large size, Ext4 allocates an additional block to 
%store the inline data. However, Ext4 forgets to clear the \textit{i\_data} field, it causes trouble 
%since Ext4 treats the i\_data as the address of indirect block when it uses direct/indirect file block 
%organization. In addition, file ACL is also stored in the extended attribute. It also attracts much 
%attention from the attackers (\texttt{CVE-2010-2946}). 


%\begin{figure}[htbp]
%	\centering
%	\includegraphics[scale=0.9]{Figures/fs-domain.pdf}
%	\caption{Vulnerability heatmap in the \textit{fs} domain}
%	\label{fig:domain}
%\end{figure}


%\textbf{Block Management (21\%).}
\noindent
\textbf{\texttt{F10:} Block management incurs an increased number of \textit{fs} vulnerabilities (21\%).} 
File systems adopt various strategies to organize file blocks. Conventional \textit{fs} like Ext2/Ext3 
use \textit{direct/indirect} block to organize file blocks. Currently, popular \textit{fs} (e.g., Ext4 and 
BtrFS) uses \textit{extents} to manage file blocks. Although extent-based \textit{fs} manages file blocks efficiently, 
our study shows that extent management is much more error-prone than direct/indirect 
block organization due to the increased complexity of block management.  
%Their causes are diverse, including improper extent operation, race condition, 
%and integer overflow. 
Take Ext4 for example, it supports both extent-based and direct/indirect block organization. 
%As developers take great effort to develop extent management, 
The codebase size  
(7K lines of codes) of the extent management is much larger than that of direct/indirect block organization (1.5K lines of codes). 
Such complexity generates more security issues (9$\times$) 
than direct/indirect block organization. 
As more features are integrated, such as flexible block group~\cite{flexblock} and 
delay block allocation, they introduce more vulnerabilities. 
We summarize them in Table~\ref{tab:fs-feature}. 
%Ext4 file system has added numerous new properties, 
%such as flexible/metadata block group, and delay block allocation. 
%%However, these newly-added 
%%features also cause severe security issues, leading to a vulnerable file system.

\begin{comment}
\begin{table}[t]
    \footnotesize
        \caption{The most vulnerable \textit{fs} components in Linux.}
        \vspace{-2ex}
    \label{tab:domain}
    \centering
	\begin{tabular}{m{60pt}<{\raggedleft}|p{15pt}<{\raggedright}|m{65pt}<{\raggedleft}|p{15pt}<{\raggedright}}
                \hline
		\textbf{FS Component} & \textbf{\%} & \textbf{FS Component} & \textbf{\%} \\
        \hline
		Inode management                    & 39\%  & Block management & 21\%\\
		Permission model                     & 14\% & Page Cache & 12\%\\
        \hline
        %\textbf{Total} & \multicolumn{3}{r}{157}\\
       % \hline
    \end{tabular}
        \vspace{-4ex}
\end{table}

\end{comment}

\begin{comment}
%\textbf{File Permission Model (14\%).}
\ben{I think we don't clearly answer the question of why this is a problem of lacking a formal specification. I'm looking for an example to help showcase this.}
\noindent
\textbf{\texttt{F12:} Most file systems lack formal specifications for their permission models (14\%).} 
\ben{I think this description (first three sentences) may be more useful the first time we mention permissions in the permission bypass section.}
File system permission model restricts the file access for users. Currently, 
it has two types: (1) traditional file permission, 
i.e., \texttt{u/g/o:r/w/x}; (2) POSIX access control list (ACL).
%\begin{inparaenum}[(\roman{enumi})]
%	\item traditional file permission, i.e., \texttt{u/g/o:r/w/x};
%	\item POSIX access control list (ACL).
%\end{inparaenum}
Almost all \textit{fs}-related system calls require correct file access restriction. 
As confirmed in $\S$~\ref{sec:cause}, most of these vulnerabilities 
are caused by the missing and insufficient permission checks. 
 Adversaries could exploit these vulnerabilities to bypass the  
access permissions and gain unauthorized kernel privileges. 
\ben{I'm not sure what is trivial about the vulnerability here, @Jian, could you clarify?} 
Although this type of vulnerability is trivial, we find that a large number of 
\textit{fs} functions suffer from this type of security issue.
%Most importantly, 
We also identify that current file systems do not have rigorous 
and formal specification for the permission model. System developers must  
manually perform permission checks on the system-call execution path to 
enforce the permission model. Inevitably, 
developers could miss or perform insufficient permission checking. 
%For example, system call like \texttt{ioctl} is specific to the file system implementation and it usually consists of a large number of case conditions and execution paths. In addition, there is no concrete documentation for such type of system call. As a result, file permission model during \textit{ioctl} execution path is error-prone and vulnerable.
\end{comment}

%\textbf{Page Cache (12\%).}
\noindent
\textbf{\texttt{F11}: Page cache and its data persistence incur \textit{fs} vulnerabilities for data leakage (12\%).} 
Modern \textit{fs} uses a page cache to improve application performance. 
%File system metadata such as \texttt{super block} are buffered in the page cache to accelerate the block accesses. Consequently, almost all file system operations load or store their requested blocks in the page cache. Even page cache could greatly boost the file system performance. Unfortunately, our study shows that page cache also introduces a security issue, i.e., uninitialized data leakage (e.g., \texttt{CVE-2005-0400}).
Specifically, the page cache usually stores metadata blocks temporarily. File systems will flush 
these metadata blocks to the underlying device via \textit{fsync}-based system calls. 
However, if system developers do not initialize certain fields of metadata structure in the page cache, 
these uninitialized data structures that contain the kernel sensitive information, will be persisted 
to the underlying persistent storage. Thus, a malicious user can obtain sensitive data 
via reading the raw device, and leverage kernel information to perform further attacks (e.g., 
\texttt{CVE-2005-0400}).

%\begin{figure}[htbp]
%	\centering
%	\includegraphics[width=\linewidth]{Figures/page-cache.pdf}
%	\caption{Comparison of two kernel data leakage}
%	\label{fig:page-cache}
%\end{figure}

%Such data leakage vulnerability is different from the kernel data leakage studied in previous paper~\cite{lu-ccs16}. In particular, there are several differences between these two types of data leakage vulnerabilities, as shown in the Figure~\ref{fig:page-cache}. First, file systems adopt a radix tree to organize these buffered metadata blocks. The basic unit stored in the radix tree is \emph{page}, which is managed by the kernel memory \emph{buddy allocator}. A single page could store several metadata blocks which depends on the size of the file system block. In contrast, the leak source of previous data leakage vulnerability is the \emph{slab}-based memory allocator. Then, Linux kernel uses the \textit{buffer\_head} data structure to describe the buffered block in the page cache. The field \textit{b\_data} in the \textit{buffer\_head} records the start offset in the page cache page. To write the corresponding data fields, file systems have to perform a type casting for \textit{b\_data} pointer and then fill the corresponding data field. On the other side, as \textit{slab} is an object-based allocator, it does not require typecasting before data write. Finally, page cache leaks the data via the file system flush system calls. Previous data leakage sinks are determinate system functions, such as \textit{copy\_to\_usr}, \textit{sock\_sendmsg} etc. As a result, prior tools~\cite{lu-ccs16} is applicable to detect data leakage vulnerabilities in page cache component.




\noindent
\fcolorbox{black}{Gray}{\parbox[c]{8.1cm}{
\textbf{Summary:}\emph{
	We identify that \textit{fs} vulnerabilities center around index management, block management, and page cache. 
	And index management is the most vulnerable component. 
	%which occupies 39\% of the total vulnerabilities.
        }
}}
\vspace{-2.5ex}

%\begin{framed}
%\vspace{-1.5ex}
%\noindent
%\textbf{Finding:}{\emph{
%	We identify that \textit{fs} vulnerabilities center around metadata management and data access 
%	permission checking. Particularly, 
%	metadata management is the most vulnerable component in file systems, which 
%	occupies 74\% of the total studied vulnerabilities.
%%Most vulnerabilities exhibits strong relation with its specific \textit{fs} component. Thus, studying these vulnerabilities in component fashion could help us fully understand the root cause of these vulnerabilities. Unfortunately, most \textit{fs} semantic bugs are unable to be detected by existing bug-finding tools.
%}}
%%\vspace{-1ex}
%\vspace{-1.5ex}
%\end{framed}
%


%
%\begin{table*}[t]
%    \footnotesize
%    \caption{Finding of mobile \textit{fs} vulnerabilities. In the fourth column, we present the distribution of the major consequences. \texttt{D:} DoS, \texttt{L:} Data Leakage, \texttt{P:} Privilege Escalation, \texttt{A:} Access Permission Bypass. }
%    \label{tab:mobifs-summary}
%        \vspace{-3ex}
%    \centering
%    \begin{threeparttable}
%    \begin{tabular}{m{30pt}<{\raggedleft}|p{105pt}<{\raggedright}|p{40pt}<{\centering}|p{90pt}<{\raggedright}|p{90pt}<{\centering} |p{40pt}<{\centering}|p{15pt}<{\centering}}
%    \hline
%    \textbf{Name} & \multicolumn{1}{c|}{\textbf{Description}} & \makecell{\textbf{Release}\\\textbf{Date}} & \makecell{\textbf{Consequences}\\($\,\,$\texttt{D}$\,\,$, \texttt{L}$\,\,$, \texttt{P}$\,\,$, \texttt{A}$\,\,\,$)} & \textbf{Attack Vector} & \makecell{\textbf{Privacy}\\\textbf{Breaches}} & \textbf{\#CVEs} \\
%
%    \hline
%            HFS/HFS+            & Hierarchical file system              & 1985  & \texttt{D}:71\%, \texttt{L}:5\%, \texttt{P}:14\%, \texttt{A}:10\%
%                        & physical:62\%, remote:38\%  &  53\% & 21 \\
%    APFS                        & Apple file system                                     & 2016  & \texttt{D}:40\%, \texttt{L}:40\%, \texttt{P}:20\%
%                                & physical:60\%, remote:40\%  & 100\% & 5 \\
%    F2FS                        & Flash-friendly file system                    & 2012  & \texttt{D}:83\%, \texttt{P}:17\%
%                                & physical:50\% remote:50\%  & 35\% & 21 \\
%    eCryptFS        & Disk encryption file system           & 2006 &  \texttt{D}:50\%, \texttt{L}:17\%, \texttt{P}:33\%
%                    & physical:83\% remote:17\% & 75\% & 12 \\
%    Others              & proc, sysfs, Ext4, debugfs, etc       &               & \texttt{D}:38\%, \texttt{L}:24\%, \texttt{P}:38\%,
%                                & physical:55\% remote:45\%  & 89\% & 9 \\
%    \hline
%    \textbf{Total} & \multicolumn{6}{r}{68}                             \\
%    \hline
%    \end{tabular}
%%    \begin{tablenotes}
%%    \scriptsize{\item[1] DoS \item[2] Data Leakage \item[3] Privilege Escalation \item[4] Access Permission Bypass}
%%    \end{tablenotes}
%    \end{threeparttable}
%	\vspace{-3ex}
%\end{table*}
%

\begin{figure*}[t]
        \centering
        \begin{minipage}[c]{\linewidth}
                \includegraphics[width=0.98\linewidth]{Figures/bug-to-security.pdf}
                %\vspace{-3ex}
        \end{minipage}
        %\vspace{-1ex}
        \caption{Percentage of \textit{fs} bugs that lead to security vulnerabilities.
        We manually study 1,311 \textit{fs} bugs totally, in which 33.0\% are sanity checking bugs,
        24.6\% are concurrency bugs, 17.8\% are memory bugs, and 11.9\% are permission bugs.
        }
        \label{fig:kernelbug}
        \vspace{-3ex}
\end{figure*}


\subsubsection{Exploiting Unique FS Features}
\label{subsec:fsfeature}
%According to our study, 
%We find that 
Adversaries also usually exploit \textit{fs} features such as crash-consistency models and virtual \textit{fs} (VFS) to initiate attacks.
%In this section, we use two case studies to demonstrate how adversaries could exploit 
%\textit{fs} features to facilitate their attacks.
%We report the top three most popular \textit{fs} features exploited by adversaries.  
%to initiate attacks, %we use case studies to demonstrate them as follows. 



%\subsection{Namespace Management}
%File system adopts a tree-like hierarchy to organize file name. Virtual file system also supports multiple namespaces in the file system.

%delay umount and bind mount contribute 33\% in namespace vulnerabilities.

%multiple namespaces require permission isolation during mount propagation.

%\textbf{Crash-safety Model.}
\noindent
\textbf{\texttt{F12:} Adversaries often exploit crash-consistency models for persistent storage to obtain sensitive kernel information.} 
Crash consistency models like journaling~\cite{ext3}, logging~\cite{log-structuring}, 
shadow paging~\cite{WAFL} are widely used in file systems. Take JFS as an example, 
%it is a typical journaling file system, its log strategy ensures that any operations performed on the metadata 
%must be consistent after system crashes. Therefore, 
it employs a synchronous writing strategy to log the storage operations and \texttt{inode}. 
%Attackers could exploit the vulnerability in JFS to obtain the kernel information (\texttt{CVE-2004-0181}). 
%Specifically, 
As JFS logs all relevant in-memory data structures, some of them may not be properly initialized/cleaned. 
Attackers can obtain sensitive kernel information by reading the raw device directly (e.g., 
\texttt{CVE-2004-0181}).
In addition, 
%we find that vulnerability occurs when the crash-safety model does not cooperate 
%well with other OS components like I/O scheduler (e.g., \texttt{CVE-2017-7495}). 
%For example, Ext4 adopts block delay allocation to improve the performance of extent management. 
%Even ext4 flushes the data blocks when it allocates the corresponding extent. However, 
%it does not add the corresponding inode block to the JBD2 transaction flush list. Unfortunately, 
%For example, 
the I/O scheduler may reorder inode block and data block. 
As a result, the inode block may come to the disk before the data block, which violates 
the \textit{ordered} journal model of JBD2. In this case, malicious users may read  
stale data from disk, which could include other users' file content (e.g., \texttt{CVE-2017-7495}). 

%As discussed, modern file systems use a page cache to improve application performance. They cache data blocks
%in the page cache for accelerating file accesses. 
%However, 
Handling the consistency between memory states and disk states is not only for ensuring  
crash safety but also for alleviating \textit{fs} vulnerabilities. 
%We need to carefully handle the consistency between memory states and disk states to avoid 
%\textit{fs} vulnerabilties. 
For instance,  
%We observe that page cache could be exploited by
%attackers to corrupt the disk data. For example, as reported in \texttt{CVE-2015-8839},
%%(see Figure~\ref{fig:CVE-2015-8839}),
Ext4 provides \textit{hole punching} to remove a portion of a file without changing its size.
To fulfill this, the corresponding data blocks residing in the page cache will be freed.
However, Ext4 does not synchronize the page fault and hole punching procedure, %leading to a race condition. In this case, 
the page fault handler would map the pages containing the data of blocks that are being freed into
another process's address space. Thus, disk data corruption and data leakage would happen, 
if these pages are written to disk (\texttt{CVE-2015-8839}). 





\noindent
\textbf{\texttt{F13:} The mismatch between VFS semantics and \textit{fs} implementations introduces vulnerabilities.} 
%\ben{(from reviewer) elaborate on why the attack surface is large}
VFS provides the general data structures and interfaces for underlying \textit{fs} 
implementations. Each specific \textit{fs} implementation must obey the VFS specification. 
However, VFS is one of the most exploitable \textit{fs} features.  
%because of three reasons. 
%First, it provides the userspace with a system call interface to access underlying file systems. 
%Second, the virtual memory manager interacts with the VFS to write data to storage. Third, 
%the VFS provides the internal low-level interface for the underlying file systems. 
We study their attack models and find that 
60\% of them are triggered via system calls (\texttt{CVE-2010-4250}, 
\texttt{CVE-2016-6516}), and 40\% of them are caused by the underlying 
\textit{fs} implementation interacting with the VFS (\texttt{CVE-2014-8559}, \texttt{CVE-2018-13405}).

%(Table~\ref{tab:vfs-cve-corr}).
Specifically, we find that there are many semantic mismatches between VFS and underlying \textit{fs} 
implementations (e.g., \texttt{CVE-2016-6198}). %\texttt{CVE-2008-3275}). 
%For example, 
%if a file is renamed to a hardlink, POSIX specifies that \texttt{rename} should do nothing and 
%return \texttt{success}. However, this condition is checked in \textit{vfs\_rename} in VFS. 
%Unfortunately, it will not detect hard links on OverlayFS, in which different OverlayFS layer has 
%separate inodes. OverlayFS itself detects this condition and returns \texttt{success} 
%without doing anything, but \textit{vfs\_rename} will proceed as if this is a successful \texttt{rename}. 
%Consequently, it would cause the system crash.
%\ben{TODO: I can update this. This example is confusing} 
For example, %if a file is renamed to a hardlink of itself, 
%POSIX specifies that \texttt{rename} should do nothing and return \texttt{success}. 
the underlying implementation of VFS -- OverlayFS unifies multiple file systems 
and provides a hierarchical namespaces~\cite{overlayfs}. 
%Different OverlayFS layer has different inode for the same namespace. 
Suppose a file is renamed to a hardlink of itself with \textit{vfs\_rename},  
%these two links could give separate inodes for different OverlayFS layer. 
VFS must retrieve the real inode via \textit{d\_select\_inode}.  
%during the \textit{vfs\_rename} procedure. 
Otherwise, VFS may proceed with an incorrect inode, resulting in 
data loss. This suggests that we need to enforce the consistent 
assumptions and implementations from the VFS to underlying \textit{fs}. 
%if the VFS does not realize it and proceeds 
%to execute \textit{d\_move} in \textit{vfs\_rename}, it would cause DoS.

%\textbf{\begin{table}[t]
%    \footnotesize
%	\caption{CVEs caused by components interacting with VFS}
%	\vspace{-1ex}
%    \label{tab:vfs-cve-corr}
%    \centering
%    \begin{tabular}{p{75pt}<{\raggedleft}|p{75pt}<{\centering}}
%		\hline	
%		\textbf{Component} &  \textbf{\% of CVEs caused}\\
%		\hline
%       	Memory Manager & 6.67\% \\
%        File Systems & 33.33\% \\
%        System Calls & 60.00\% \\
%        \hline
%   \end{tabular}
%	\vspace{-2ex}
%\end{table}}


%\begin{table}[t]
%    \footnotesize
%        \caption{Defense strategies for generic \textit{fs} vulnerabilities.}
%        \vspace{-3ex}
%    \label{tab:linux-fix}
%    \centering
%    \begin{tabular}{p{8pt}<{\centering}|p{185pt}<{\raggedright}|p{15pt}<{\raggedright}}
%                \hline
%                \textbf{} & \textbf{Fixing Strategies} & \textbf{\%} \\
%        \hline
%            \multirowcell{6}{\begin{turn}{90}Sanity checking\end{turn}}
%                                             & Validate fs image before mounting &  48.2\%\\
%                                             & Enforce restrictions on the file size & 12.5\% \\
%                                             & Validate memory pointers before dereferencing & 5.4\%\\
%                                             & Check for the division by zero & 3.9\% \\
%                                            % & Check if a mount path is unmounted before using it & 3.6\% \\
%                                             & Check for integer overflows & 3.6\% \\
%                                             & Others & 26.4\%\\
%        \hline
%            \multirowcell{4}{\begin{turn}{90}Concurrency\end{turn}}
%                                            & Make ToCToU race operations atomic &  42.9\%\\
%                                            %& Initialize corruptible data copied from user-space &  14.3\%\\
%                                            %& Free the data entry before assigning a lock to it & 14.3\% \\ 
%                                            & Use of Lock-free optimizations & 28.6\% \\
%                                            & No locked data structure in fault handler & 7.2\% \\
%                                            & Others & 21.3\% \\
%        \hline
%            \multirowcell{4}{\begin{turn}{90}Mem Err\end{turn}}
%                                            %& Check for memory errors on fault-handling paths & 38.5\% \\
%                                            & Initialize unused, allocated memory & 38.5\% \\
%                                            %& Initialize unused, allocated kernel memory & 11.5\% \\
%                                            %& Prevent mount when metadata blocks overlap super blocks for a file system & 7.7\% \\
%                                            & Initialize structures before copying data from user space & 24.2\% \\
%                                            & Initialize the new group descriptor upon fs resizing & 14.3\% \\
%                                            & Others & 23.0\%\\
%        \hline
%            \multirowcell{4}{\begin{turn}{90}File Perms\end{turn}}
%                                            %& Check for user privileges for mount propagation, ACL modifications, inode encryption policy, mount flag changes, etc. & 38.1\% \\
%                                            & Check user privileges  & 42.9\% \\
%                                            & Add file permission checks for ioctl operations  & 28.6\% \\
%                                                                %& Check for \texttt{ADMIN} capabilities for mount propagation & 14.3\% \\
%                                                                %& Check user privileges before changing mount flags & 9.5\% \\
%                                                                %& Check for integer overflows in  & 9.5\% \\
%                                                                %& Check for user capabilities before allowing modifications to ACLs & 9.5\% \\
%                                          %& Check for null pointers on fault-handling paths before using them & 4.8\% \\
%                                          & Validate block group information before mounting fs  & 4.8\% \\
%                                    %& Check user capabilities before allowing set up of inode encryption policy & 4.8\% \\
%                                          & Others & 23.7\% \\
%        \hline
%    \end{tabular}
%        \vspace{-3ex}
%\end{table}
%


==> correlation.tex <==
%\vspace{-2ex}
%\section{Correlation between FS bugs and CVEs}
%\begin{table*}[t]
%    \footnotesize
%	\caption{Correlation between bugs and vulnerabilities in \textit{fs}.}
%	\vspace{-1ex}
%    \label{tab:cve-bugs-corr}
%    \centering
%    \begin{tabular}{|m{80pt}<{|\raggedleft}|p{30pt}<{\centering}|p{30pt}<{\centering}|p{30pt}<{\centering}|p{30pt}<{\centering} | p{30pt}<{\centering}|p{30pt}<{\centering}|p{30pt}<{\centering}|p{30pt}<{\centering}|}
%		\hline	
%		\multicolumn{1}{|c|}{} & \textbf{Ext2} & \textbf{Ext3} & \textbf{Ext4} & \textbf{XFS}
%		& \textbf{F2FS}
%		& \textbf{ReiserFS}
%		& \textbf{Btrfs}
%		& \textbf{JFS}\\
%       	\hline
       	
%       	{\% Bugs caused by Sanity Checking} & 23.97 & 32.33 & 34.8 & 34.72 & 24.01 & 24.94 & 24.75 & 27 \\
 %      	\hline
 %      {\% CVEs caused by Sanity Checking} & 46 & 51 & 55 & 37 & 67 & 20 & 30 & 50\\
  %     \hline
 %      {\% Sanity Checking bugs causing CVEs}	& 5.48 & 3.53 & 6.45 & 2.74 & 8.72 & 1.14 & 1.48 & 3.31\\
 %       \hline
%        {\% Bugs caused by Concurrency} & 21 & 18 & 16 & 18 & 17 & 42 & 20 & 23\\
 %       \hline
  %      {\% CVEs caused by Concurrency} & 12 & 0 & 10 & 3 & 18 & 0 & 5 & 0\\ 
%        \hline
 %       \% Concurrency bugs causing CVEs	& 1.63 & 0 & 2.55 & 0.43 & 3.3 & 0 & 0.3 & 0\\
  %      \hline
%        \% Bugs caused by Memory Errors & 16 & 8 & 14 & 10 & 15 & 8 & 10 & 22\\
  %      \hline
%        \% CVEs caused by Memory Errors	& 15 & 14 & 15 & 37 & 14 & 40 & 18 & 50\\
 %      \hline
%         \% Memory bugs causing CVEs & 2.68 & 3.92 & 4.37 & 9.5 & 2.92 & 7.12 & 2.2 & 4.06\\
  %       \hline
%        	\% Bugs caused by File Permissions	& 16 & 13 & 10 & 10 & 19 & 7 & 15 & 10\\
 %       	\hline
  %      	\% CVEs caused by File Permissions & 12 & 10 & 5 & 3 & 4 & 20 & 25 & 0\\
%        	\hline
  %      	\% File Permission bugs causing CVEs & 2.14 & 1.72 & 2.04 & 0.77 & 0.66 & 4.07 & 2.04 & 0 \\
% 	    \hline
 %       	\% Bugs caused by Other Errors	& 23.03 & 28.67 & 25.2 & 27.28 & 21.62 & 18.06 & 30.25 & 18\\
   %     	\hline
    %    	\% CVEs caused by Other Errors	& 15 & 25 & 15 & 20 & 5 & 20 & 22 & 0\\
    %    	\hline
%        	\% Other bugs causing CVEs & 1.86 & 1.95 & 2.43 & 1.88 & 0.72 & 1.58 & 0.89 & 0\\
  %      	\hline
%        	\textbf{Total \% of bugs that cause CVEs} & \textbf{2.86} & \textbf{2.24} & \textbf{4.08} & \textbf{2.57} & \textbf{3.12} & \textbf{1.42} & \textbf{1.22} & \textbf{1.79} \\
%        \hline
%    \end{tabular}
%	\vspace{-4ex}
%\end{table*}



==> dfs.tex <==
\begin{table*}[t]
    \footnotesize
    \caption{Distribution of networked \textit{fs} vulnerabilities. In the fourth column, we present the distribution of the major attacks: {D:} DoS, {L:} Data Leakage, {E:} Privilege Escalation, {A:} Access Permission Bypass. In the fifth column, we present the correlation threats: {Local:} correlation with local FS or OS; {CollocatedFS:} correlation with collocated FS instances.}
    \label{tab:dfs-summary}
        \vspace{-2ex}
    \centering
    \begin{threeparttable}
    \begin{tabular}{|m{30pt}<{\raggedleft}|p{120pt}<{\raggedright}|p{30pt}<{\centering}|p{115pt}<{\raggedright}|p{115pt}<{\raggedright} |p{20pt}<{\centering}|}
    \hline
    \textbf{Name} & \multicolumn{1}{c|}{\textbf{Description}} & \makecell{\textbf{Release}\\\textbf{Date}} & \makecell{\textbf{Consequences}\\($\,\,${D}$\,\,$, {L}$\,\,$, {E}$\,\,$, {A}$\,\,\,$)} & \textbf{Correlation Threats}  & \textbf{\#CVEs} \\

    \hline
    NFS  & Networking File System              & 1984  & 
    {D}:\colorbox{pink}{68\%}, {L}:1\%, {E}:12\%, {A}:18\% & Local:\colorbox{pink}{27\%}, CollocatedFS: 2\% &   72 \\
    OpenAFS  & An open source release of the AFS & 2016  &  {D}:\colorbox{pink}{63\%}, {L}:\colorbox{pink}{30\%}, {E}:4\%, {A}:4\%  & {Local}:\colorbox{pink}{26\%}, {CollocatedFS}: 0\% &  27 \\
    CephFS  & A distributed object storage platform    & 2006  & {D}:\colorbox{pink}{73\%}, {L}:20\%, {E}:7\%, A:0\%   & {Local}:\colorbox{pink}{21\%}, {CollocatedFS}: 0\%  & 19 \\
    GlusterFS  & A scalable network filesystem    & 2005  & {D}:\colorbox{pink}{28\%},  {L}:17\%,  {E}:17\%, {A}:\colorbox{pink}{38\%}  & {Local}:\colorbox{pink}{11\%}, {CollocatedFS}: \colorbox{pink}{6\%} &  18 \\
%    GPFS			& IBM General Parallel File System &1998 &  {D}:\colorbox{pink}{29\%}, {L}:21\%, {E}:\colorbox{pink}{43\%}, {A}:7\%   & No reported CVE cases & 14\\
    HDFS	   		& Hadoop Distributed File System & 2011 & {D}:\colorbox{pink}{33\%}, {L}:17\%, {E}:\colorbox{pink}{33\%}, {A}:17\%  & No reported CVE cases & 6\\

%    \hline
%    \textbf{Total} & \multicolumn{6}{r}{68}                             \\
    \hline
    \end{tabular}
%    \begin{tablenotes}
%    \scriptsize{\item[1] DoS \item[2] Data Leakage \item[3] Privilege Ecalation \item[4] Access Permission Bypass}
%    \end{tablenotes}
    \end{threeparttable}
        \vspace{-4ex}
\end{table*}


% this table mingles attacks with consequences and duplicates with table 2 and 8.
% and the categories somehow overlap
\begin{comment}
\begin{table}[t]
    \footnotesize
	\caption{Major attacks in networked \textit{fs}.}
	\vspace{-2ex}
    \label{tab:dfs-cause}
    \centering
    \begin{tabular}{|r|p{120pt}<{\raggedright}|}
		\hline		
		\textbf{Attack}  & \textbf{Description} \\
        \hline
	    \multirow{2}{*}{Networking (25\%)} 		 & Mishandle HTTP package (35\%) \\
       							 & Mishandle RPC package (63\%) \\
       	\hline
        \multirow{1}{*}{Remote ACL (20\%)}   & Remote ACL (39\%) \\
        \hline
        Authentication (12\%)	& Privilege escalation \\
        \hline
	    Concurrent Data Access (4\%) & Mishandle concurrent file accesses \\
	    \hline
    \end{tabular}
	\vspace{-4ex}
\end{table}
\end{comment}


%\begin{figure}[t]
%\centering
%\begin{minipage}[c]{110pt}
%	\centering
%	\includegraphics[width=0.98\textwidth]{Figures/dfs_cause.pdf}
%\subcaption{Causes}
%\label{fig:dfs-cause}
%\end{minipage}
%\begin{minipage}[c]{128pt}
%	\centering
%	\includegraphics[width=0.98\textwidth]{Figures/dfs_consq.pdf}
%\subcaption{Consequences}
%\label{fig:dfs-conseq}
%\end{minipage}
%	\vspace{-3ex}
%	\caption{Causes and consequences distribution of networked \textit{fs} vulnerabilities.}
%	\vspace{-3ex}
%\end{figure}


\section{Networked FS Vulnerability}
\label{sec:dfs}
Beyond generic \textit{fs} ($\S$~\ref{sec:genericfs}) and mobile \textit{fs} ($\S$~\ref{sec:mobilefs}), 
we also study the networked \textit{fs} vulnerabilities. 
In this paper, the \textit{networked fs} refers to the \textit{fs} instances connected 
with networking, such as NFS~\cite{nfs}, and HDFS~\cite{hdfs}. %which includes the distributed file systems and networking file systems. 
As we expected, similar attacks identified in the generic \textit{fs} also appear in the 
networked \textit{fs}. However, we are more interested in the \textit{fs} vulnerabilities that 
are unique to the networked environment. 


%\subsection{Causes and Consequences}
We examine 142 vulnerabilities in six widely-used networked \textit{fs} as shown in Table~\ref{tab:dfs-summary}. 
Besides the attacks discussed in $\S$~\ref{sec:cause}, we identify another three types of attacks unique to the networked \textit{fs}. 
%as described in Table~\ref{tab:dfs-cause}. 
They include the networking vulnerability, 
and the vulnerabilities related to authentication and remote ACLs.
Similar to generic and mobile \textit{fs}, DoS is the major attack (57\% on average) in networked \textit{fs} in general (see Table~\ref{tab:dfs-summary}). 
However, we observe that DoS attack is becoming less popular, while data leakage deserves more attentions recently, as shown in Figure~\ref{fig:dfsattacktrend}. 
%Furthermore, we examine how network \textit{fs} vulnerabilities are correlated with local or remote \textit{fs} 
%instances. 
%We show their distribution across networked 
%\textit{fs} in Figure~\ref{fig:dfs-cause}.
%We also present the distribution of the consequences caused by networked \textit{fs} vulnerabilities  
%in Figure~\ref{fig:dfs-conseq}. 
%We find that the networking and authentication vulnerabilities are prevalent in networked file systems. 



%
%\begin{table}[t]
%    \footnotesize
%	\caption{Major causes of networked \textit{fs} vulnerabilities.}
%	\vspace{-3ex}
%    \label{tab:dfs-cause}
%    \centering
%    \begin{tabular}{p{75pt}<{\centering}|p{40pt}<{\raggedright}|p{100pt}<{\raggedright}}
%		\hline		
%		\textbf{Cause} & \textbf{Sub-type} & \textbf{Description} \\
%        \hline
%	    \multirowcell{2}{Networking (47\%)} 		& HTTP error & Mishandle \texttt{http} package \\
%       							&  RPC error & Mishandle RPC package \\
%       	\hline
%       	Authentication (33\%)				 	& N/A & Authentication error \\
%        \hline
%       	\multirowcell{2}{Remote ACL (20\%)} 	& Miss perm & Miss permission checking \\
%       								 	& Inapt perm & Improper permission checking \\
%        \hline
%    \end{tabular}
%	\vspace{-3ex}
%\end{table}
%




\jinghan{The numbers in Table 2, Table 8, and this section are consistent with the updated dataset;}
\subsection{Common Attacks in Networked FS}
\label{sec:networked}
%\ben{Reviewer C did not find this section compelling} 
We present the common attacks in networked \textit{fs} in Figure~\ref{fig:dfsattack}.
%to facilitate our characterization study. 
%\noindent
%\textbf{\texttt{F20:} Networking management is on the critical path of ensuring the safety of networked \textit{fs}.} 
In networked \textit{fs}, the networking management involves both data transfer (via HTTP and RPC) and access authentication. 
Adversaries usually exploit the vulnerabilities in the network packet transfer and processing to initiate their attacks. 
Unlike generic and mobile \textit{fs}, networked \textit{fs} usually relies on remote ACLs to enforce 
the access control of distributed files. 
%A common attack approach is to exploit the vulnerabilities in the 
%\textit{fs}-specific service protocols like the Service Level Authorization used in HDFS~\cite{hadoop-auth}, 
%and ACL management daemon running on the storage servers.
%The attack model analysis helps us pinpoint the 
%most vulnerable components in networked \textit{fs}. We will discuss each of them as follows.  

%\subsection{Networking Flaws}
%\subsection{Interactions with Networking Protocols}
%\label{sec:net}
%\jinghan{Reviewer E: Section 5.2 seems misnamed. It's not a flaw with networking. It seems to be flaws with how the file system interacts with RPC and HTTP networking protocols. Please say that clearly.}
\noindent
\textbf{\texttt{F20:} A significant portion (63\%) of networking flaws (25\%) are exploited by crafted RPC to launch DoS attacks.}
Networked \textit{fs} is utilizing various networking protocols to perform the 
identity verification, file transfer, and data recovery. Typical protocols include HTTP and RPC. 
The vulnerabilities found in these protocols pose great threats to networked \textit{fs}. 
%We find that these networking issues contribute to 39\% of the networked \textit{fs} vulnerabilities. 
And most vulnerabilities (e.g., \texttt{CVE-2015-5245}) 
%\texttt{CVE-2016-8626}, \texttt{CVE-2018-7262}) 
happened due to the mishandling of malformed or crafted network packets, such as zero payloads, 
crafted packet header, and uninitialized packets. 
Attackers can exploit these flaws to inject malicious code and hijack the critical workflow. 
%\jinghan{On the contrary, only few vulnerabilities require attackers to gain access to the server nodes and attack as local users (5.8\% in Ceph, 14.2\% in HDFS), which are often more difficult to be exploited than networking flaws. They mostly attack through memory management flaws and result in DoS. Therefore, we believe that networked file system developers should put more focus on protecting the integrity of networking and remote ACL protocols.}

%and even compromise the whole networked system.

Specifically, RPC protocol is widely used in networked \textit{fs} for accessing remote files.
We find that a significant number 
of RPC-related vulnerabilities are caused by the 
mishandling of RPC packets (e.g., \texttt{CVE-2003-0576}, \texttt{CVE-2018-16949}). 
Some of them can be exploited by attackers to conduct DoS and privilege escalation attacks. 
For example, since GlusterFS allows RPC request to create symlink (e.g., \texttt{gfs3\_symlink\_req}) 
pointing to file paths in the GlusterFS volume, remote attackers can exploit this to 
send crafted RPC to create arbitrary symlinks in the storage server and then execute arbitrary 
code (e.g., \texttt{CVE-2018-10928}).   
%RPC-related vulnerabilities may trigger buffer overflow at first (e.g., \texttt{CVE-2013-1795}), and 
%then indirectly cause DoS attack.


%\noindent
%\textbf{\texttt{F24:} RPC-related vulnerability is a major contributor to the DoS attacks by over-consuming 
%the system memory.} For example, the RPC uses external data representation (XDR) to marshall 
%and unmarshall the stream of data over the network. However, 
%%the marshalling and unmarshalling 
%they happen before the sanity checking of RPC procedures. 
%Therefore, attackers can bypass the checking and keep sending malicious requests with an 
%XDR unbounded array type to exhaust the memory available on the server. 
%After that, the server fails to respond to other legal memory requests (e.g., \texttt{CVE-2018-16949}). 
%%A communication flaw can also be leveraged by adversaries to perform code reuse attack. For example, 
%%as reported in \texttt{CVE-2015-7762}, 
%%when the client sends a RPC request to the server to query attribute or state information, 
%%the corresponding data structure such as \texttt{VldbListByAttributes} that needs to be filled. 
%%%These leaked data may come from 
%%This may leak the information of the userspace stack or even the kernel memory. 
%%With sniffing the network packets, attackers can obtain the sensitive information. 
%%%such as memory layout of the kernel or user process. 
%%%It may cause some valuable pointer information of the client process may leaked to the attacker. 
%%As a consequence, the attack may use these pointer to bypass the ASLR, leading to a code-reuse attack.
%%Moreover, remote attackers can execute privilege escalation attack by exploiting 
%%the RPC-related vulnerabilities. 
%


\noindent
%\textbf{\texttt{F24:} Flaws in HTTP communitation contributes to significant portion (24\%) of networking-related vulnerabilities.}
\textbf{\texttt{F21:} Adversaries usually exploit HTTP flaws (35\% of networking attacks) to initiate code injection attacks in networked \textit{fs}.} 
%We find that adversaries usually exploit HTTP flaws to issue code injection attacks. 
%According to our study, such vulnerabilities occupy 24\% of the networking flaws. 
%\ben{Reviewer A: ``it should be noted that RGW in Ceph is not a file system, its an object storage with a REST API. Not to be mixed with CephFS"} 
Take the CephFS as an example, it uses the Ceph Object Gateway daemon (RGW) as an HTTP server to 
communicate with Ceph storage cluster and retrieve file data. 
%Take the Ceph Object Gateway daemon (RGW) as an example, RGW is an HTTP server which communicates 
%with Ceph Storage Cluster to retrieve file data. 
Adversaries can exploit HTTP response splitting (HRS) flaw in the RGW to initiate the 
well-known Carriage Return Line Feed (CRLF) injection and cross-site scripting (XSS) 
attack (e.g., \texttt{CVE-2015-5245}). Since the RGW does not filter the malicious carriage 
return in the HTTP requests, %when transferring a bucket name, 
attackers can exploit this CRLF injection vulnerability to send a HTTP request with a crafted bucket name. 
Once the malicious code is injected, attackers will have the privilege escalation 
to compromise the victim server, and then tamper the entire networked storage cluster.
%To mitigate this vulnerability, RGW needs to sanitize the HTTP header.  
%when including it into the HTTP request.



%\textcolor{red}{
%Replay attack could be happened due to two vulnerabilities of RPC implementation in OpenAFS (\texttt{CVE-2015-7762}, \texttt{CVE-2015-7763}). These two flaws in RPC acknowledgment (ACK) cause certain octets uninitialized due to compiler error and bugs in path MTU implementation respectively. Further, the OpenAFS adopts a per-process pool for packet buffer. These packets would not be initialized or cleared when they are put into and pulled from the pool. It results in these uninitialized octets reveal the packet data that recently be decrypted. The attacker would perform a replay attack by sending a deplicate packet to the recipient. Consequently, the attack would obtain the decryped packet data via the returned ACK packet.
%}



\noindent
\fcolorbox{black}{Gray}{\parbox[c]{8.1cm}{
\textbf{Summary:}\emph{
In networked \textit{fs}, adversaries usually exploit vulnerabilities in the
networking protocols, such as RPC and HTTP, to initiate their attacks.
        }
}}


%\subsection{Authentication and Remote ACL}
%\label{sec:auth}
\noindent
\textbf{\texttt{F22:} Adversaries often exploit the vulnerabilities in the handling of credential messages in the authentication component to achieve privilege escalation (12\%) in networked \textit{fs}.} 
Authentication protocol provides secure networking communication. 
It has been widely used in modern networked \textit{fs} to certify users, when they 
issue I/O requests. Current networked \textit{fs} either develops its   
own authentication protocol~\cite{weil2006ceph} or delegates it to the third-party 
infrastructure~\cite{steiner1988kerberos, pawlowski1994nfs}.
When vulnerabilities happen during the identity verification, attackers can 
easily trick the authentication server and bypass the access restrictions. 
We find a large number of such cases %(24\% of the vulnerabilities in networked \textit{fs} on average) 
in Ceph and HDFS. And most vulnerabilities happen,  
because networked \textit{fs} mishandles the user credential messages. For example,  
After missing the validation of the entire blocks during the signature check,   
% (2) enforcing capabilities for Ceph pool operations incorrectly. 
%Afterwards, 
clients are allowed to perform unauthorized operations like deleting system snapshot images, 
which causes data loss and leakage. 
This is true even though networked \textit{fs} uses third-party authentication platform like 
Kerberos~\cite{steiner1988kerberos}. 
Typical examples include using weak encryption (DES) for Kerberos keys (\texttt{CVE-2013-4134}), 
and mishandling Kerberos credential cache (\texttt{CVE-2009-3516}). 

%To further enhance the security of authentication, a hybrid approach has been adopted in some 
%distributed file systems such as HDFS. However, similar security vulnerabilities have been identified 
%in this approach. Take the HDFS as an example, if a DataNode registers a block pool more than 
%once with the NameNode, it would never check the BlockToken validation sent by clients. Attackers 
%can exploit this to bypass the authentication to access arbitrary blocks (\texttt{CVE-2012-3376}). 

\noindent 
%\textbf{\texttt{F27:} Remote ACL mechanism are often implemented falsely.}
\textbf{\texttt{F23:} Adversaries usually take advantage of missed validation operations in remote ACL (39\% of permission attacks)
to bypass permission check (20\%).}
Beyond the authentication of user identities, networked \textit{fs} also utilizes the access control 
to validate file access request. %They usually offload the access control to file systems servers.  
Adversaries usually exploit the vulnerabilities in the access control management of remote servers 
to obtain file permissions. 
The common causes of these vulnerabilities include: 
(1) missing the validation operation before setting ACL (e.g., \texttt{CVE-2005-3623}); 
%\texttt{CVE-2016-1237}); 
(2) missing the permission checks (e.g., \texttt{CVE-2009-1630}). 
As reported in \texttt{CVE-2009-1630}, 
a trivial flaw in NFS ACL management could cause severe consequences. For example, 
%To be specific, 
attackers can leverage the vulnerability of missing the checks of the file permission 
bit \texttt{MAY\_EXEC} to execute malicious code in storage servers.  
Similar issues are also reported in \texttt{CVE-2005-3623} and \texttt{CVE-2016-1237}. 

% 4\% is aligned with Table 2
\noindent
\textbf{\texttt{F24:} Adversaries exploit flaws in the concurrency control of networked \textit{fs} to initiate DoS and data leakage attacks (4\%).} 
Networked \textit{fs} needs to handle concurrent file accesses. A common approach is to implement file locking at a block or file granularity. Remote attackers can launch DoS attacks by exploiting race conditions (e.g. \texttt{CVE-2007-6599}, \texttt{CVE-2008-4307}) and deadlocks (e.g. \texttt{CVE-2014-1453}) when multiple clients concurrently access the shared file. 
To improve the concurrent throughput, networked \textit{fs} usually offloads some functions of the file management such as file permission check to clients with read/write delegation~\cite{pawlowski2000nfs, write-delegation}. Malicious users can exploit the offloaded functions to obtain sensitive information in the back-end servers, for example, a malicious client can concurrently issue writes and reads to the same file, and obtain sensitive information in the out-of-date page cache (\texttt{CVE-2014-2038}). 

%Networked \textit{fs} have also optimized their concurrency control to achieve better performance, but they could be vulnerable to remote attackers. For example, NFS has proposed write delegation to reduce network traffic \cite{pawlowski2000nfs}. Write delegation is granted to a single client to guarantee that it has exclusive access to a file. As reported in \texttt{CVE-2014-2038}, this could cause kernel memory leakage if a client holds rite delegation but its page cache is not updated. 
%\jian{I don't understand why this is relevant to correlation. Of course, NFS needs to handle concurrent client accesses. I think the insight you want to add here is how adversaries exploit the concurrent data accesses to compromise the DFS?}
%\jinghan{Yes. I think it is more appropriate to move it to Section 5.1.}



\noindent
\fcolorbox{black}{Gray}{\parbox[c]{8.1cm}{
\textbf{Summary:}\emph{
 Although different identity authentication and access control approaches are employed in networked
\textit{fs}, data access permission 
is still a major vulnerable part. %in the system design and implementation. 
        }
}}
\vspace{-2ex}

\subsection{Correlation Threats in Networked FS}
\label{sec:correlation}
Networked \textit{fs} usually has diverse \textit{fs} instances. 
For instance, HDFS~\cite{shvachko2010hadoop} and GFS~\cite{ghemawat2003google} manage a group of 
\textit{fs} instances within a cluster of servers. Each instance runs atop the local \textit{fs} 
and delegates the local \textit{fs} to store data on the disk. Other networked \textit{fs} like 
NFS~\cite{pawlowski1994nfs} and GlusterFS~\cite{boyer2012glusterfs} implement the \textit{fs} instance with 
specific kernel modules or user-space \textit{fs}.
%To facilitate our study, 
We categorize 
them in two dimensions: 
(1) the correlation with the local \textit{fs}; (2) the correlation with remote \textit{fs} instances. 
We show their distribution in the 5th column in Table~\ref{tab:dfs-summary}.

\noindent
\textbf{\texttt{F25:} Correlation with local \textit{fs} and OS kernel.} 
A large portion of vulnerabilities in networked \textit{fs} are caused by the miscommunication with 
local \textit{fs} and OS kernel.
%According to our study, correlated vulnerabilities can be triggered due to the miscommunication with OS kernel stack.  
These vulnerabilities are hard to fix, because they are usually related to kernel semantics. 
For instance, the authentication module (CephX) in CephFS ignores the error condition, when 
invoking the memory allocation function \emph{kmalloc} (\texttt{CVE-2014-6417}). 
%as shown in Figure~\ref{fig:CVE-2014-6417}. 
A remote attacker can exploit this to crash the Ceph monitor daemon. 
To be specific, the attacker sends a long unencrypted authentication ticket with abnormal size. % in \texttt{step 1}. 
Although the kernel memory allocator returns error and fails to response the memory request, % in \texttt{step 3}, 
the CephX module does not catch this fault. Therefore, the OS kernel would hit an out-of-bounds memory access, %in \texttt{step 4}, 
leading to the kernel crash. More interesting cases include \texttt{CVE-2010-2943} and \texttt{CVE-2015-8952}. 
\jinghan{There are many motivating examples for correlated local fs vulnerabilities. CVE-2019-15538 is an example of correlation threats with local fs; CVE-2020-24394 is a case of correlated local fs ACL error; CVE-2012-4417 is another interesting symlink attack; We mentioned local fs here but all the examples are correlation with OS kernel.}
%\ben{I think the following is a good example to add or replace the previous: For instance, XFS's procedure to perform an inode lookup did not properly check whether the inode was from an external source (such as NFS). When an external inode did not appear in the inode allocation btree it would treat this as fs corruption. The existence of external inodes also meant that just checking for well formatted inodes on disk was not valid. Those checks needed to go through the allocation btree  (CVE-2010-2943). (We could also do a writeup of (CVE-2015-8952) which is another example of interactions between local and networked fs in ways not expected).}

To quantify the attack surface introduced by the correlations, we counted the number of APIs and system calls exposed to the user-space programs. 
As shown in Table~\ref{tab:attacksurface}, all networked file systems studied in this paper developed tens of functions/APIs for interacting with local \textit{fs} and OS. 
Most of these network file systems also use RPC or HTTP for communicating with other \textit{fs} instances or components. 
%Another typical correlated vulnerabilities happen when an event running in the networked 
%file system instance conflicts with an event running in the local system. 
%For instance, as reported in \texttt{CVE-2010-1087}, a malicious user can conduct DoS attacks through  
%NFS by truncating a file and issuing a non-interruptible operation (e.g., fatal signal) at the same time. 
%Specifically, the virtual memory does not allow page invalidation operation \texttt{mapping$\rightarrow$a\_ops$\rightarrow$invalidatepage} 
%to fail, however, the function \texttt{nfs\_wb\_page\_cancel} in NFS may fail because it can be interrupted by a fatal signal, 
%resulting in system crash.
%%\textcolor{red}{
%%Specifically, when NFS kernel module is waiting these invalidated page writing back, it could be interrupted by a fatal signal. Consequently, the function \texttt{nfs\_wb\_page\_cancel} in NFS may fail due to this fatal signal. However, the kernel virtual memory manager does not allow the page invalidation operation to fail. Otherwise, it would lead to kernel crash.
%%}

%%We investigated how VFS and NFS in Linux kernel interact and their vulnerabilities could be exploited.
%\noindent
%\textbf{\texttt{F28:} Correlation with VFS.} 
%%Similar vulnerabilities have been identified in NFS.     
%We find that nearly 39\% of vulnerabilities in networked \textit{fs} can be triggered through VFS, and vice versa,  
%nearly 11\% of vulnerabilities in VFS can be triggered through networked \textit{fs}. 
%%Most of the vulnerabilities in NFS that can 
%%be triggered through VFS can be triggered by local users. 
%For example, as shown in \texttt{CVE-2014-2038},  
%a write delegation from the NFS server allows local users to extend a write operation without up-to-date 
%verification, it provides the opportunity for malicious users to obtain sensitive kernel information 
%by writing a file in NFS and then reading the same file. 
%%to check if the cached pages need to be written to an NFS file, which allows local users to obtain sensitive information from kernel memory in opportunistic circumstances by writing to a file in an NFS filesystem and then reading the same file, thereby leading to a data leak.


%\begin{figure}[t]
%\centering
%	%\vspace{-2ex}
%\begin{tikzpicture}
%[
%	style1/.style={
%			circle,
%			scale=0.75,
%			draw=blue!50,
%			fill=blue!20,
%			font=\scriptsize,
%			thick},
%	style2/.style={
%			circle,
%			scale=0.75,
%			draw=cyan,
%			fill=cyan!50,
%			font=\scriptsize,
%			thick},
%	style3/.style={
%			circle,
%			scale=0.75,
%			draw=red,
%			fill=red!50,
%			font=\scriptsize,
%			thick},
%	style4/.style={
%			scale=0.75,
%			align=center,
%			rectangle,
%			dashed,
%			rounded corners,
%			minimum width=10mm,
%			minimum height=8mm,
%			draw=black
%	},
%]
%
%\draw [dashed, thick] (-2,0) -- (5,0);
%\node at (-1.5,0.5) {\scriptsize user space};
%\node at (-1.4,-0.5) {\scriptsize kernel space};
%
%\node at (0.5,0.5) [style1] (node1) {\scriptsize s1};
%\node at (1,-0.5)  [style2] (node2) {\scriptsize s2};
%\node at (2.5,-0.5)  [style3] (node3) {\scriptsize s3};
%\node at (4,-0.5)  [style3] (node4) {\scriptsize s4};
%
%\node at (1,-0.9) {\scriptsize ceph\_x\_decrypt};
%\node at (2.5,-0.9) {\scriptsize kmalloc};
%\node at (4,-0.9) {\scriptsize \textcolor{red}{memcpy}};
%\node at (2.5,-1.5) [style4] {\scriptsize \textcolor{red}{Issue:} fails due \\ \scriptsize to abnormal size};
%
%\draw [thick, ->] (node1) -- (node2);
%\draw [thick, ->] (node2) -- (node3);
%\draw [thick,dashed, ->] (node3) -- (node4);
%
%\draw [thick, dashed, ->] (0,-2)--(4,-2);
%\node at (2,-2.3) {\scriptsize Time};
%
%\end{tikzpicture}
%	\vspace{-3ex}
%\caption{Missing error handling in CephX kernel module. 
%	%Libceph issues a auth ticket request with huge size to CephX kernel module. It would leads to \texttt{kmalloc} fails and CephX does not catch this fault, causing out-of-bounds memory access.
%	}
%	\vspace{-3ex}
%\label{fig:CVE-2014-6417}
%\end{figure}

\noindent
%\textbf{\texttt{F29:} Correlation of threats exists between different \textit{DFS} service instances.}
\textbf{\texttt{F26:} Correlation with collocated \textit{fs} instances.} 
%\paragraph{Failure Isolation:}
As the number of \textit{fs} instances can be scaled up to thousands,
there is a high possibility that some storage nodes have failures. 
Networked \textit{fs} should guarantee high availability, and ensure that single-node failure does not propagate 
to other nodes. However, this is challenging in practice. 
Take GlusterFS for example, it supports \emph{brick multiplexing} to reduce memory consumption, 
which allows multiple compatible bricks to share the same process 
and manage their own data volumes. However, a \emph{NULL} pointer dereference from 
a client request %to get file content through extended attributes
(\texttt{CVE-2018-10914}) can break the brick server process. 
As a consequence, this crash will propagate to other multiplexed brick processes, resulting 
in the system crash of the entire GlusterFS.
\jinghan{Remove GPFS done.}
%Moreover, many networked file systems, such as GFS~\cite{ghemawat2003google}, adopt 
%a \textit{master-slave} architecture, in which a single master node manages multiple data nodes. 
%However, it is possible that a compromised master node will expose security threats to the entire cluster. 
%For example, two vulnerabilities occur in HDFS (\texttt{CVE-2014-0229, CVE-2016-5393}) due 
%to the lack of privilege checking. These vulnerabilities allow unauthorized clients to 
%leverage NameNode to perform privileged operations, causing DataNode shutdown and data los
%Attackers could exploit such vulnerabilities to execute DoS attack (e.g., \texttt{CVE-2017-1304}).s.


\noindent
\fcolorbox{black}{Gray}{\parbox[c]{8.1cm}{
\textbf{Summary:}\emph{
 As networked \textit{fs} is complicated, correlated vulnerabilities are potentially becoming a big security threat. 
 Most of them are caused by the misuse of
the interfaces, mechanisms, and policies provided by the underlying \textit{fs}.
        }
}}

\vspace{-2ex}


%\subsection{Correlation with Generic File Systems}
%
%As Table~\ref{tab:dis-mobile-gen} shows, nearly 60\% or more vulnerabilities in generic, mobile and distributed file systems lead to denial of service(DoS). The average severity, impact and exploitability levels are medium (with scores greater than 3.9) for vulnerabilities across the board, with an exception being distributed file systems which level of exploitability and average score of 7.5 (Table~\ref{tab:dis-mobile-gen}). Also, Table~\ref{tab:dis-mobile-gen} shows that across all types of file systems, most of the vulnerabilities have medium levels of severity (generic: 66\% and distributed: 61\%) and impact (generic: 48\% and distributed: 46\%). 
%
%Despite of a some similarities, these file systems also have key differences. As noted above, vulnerabilities in distributed file systems are more exploitable than those in generic file systems, primarily because nearly 61\% its vulnerabilities can be exploited remotely, most of which can be exploited from the aforementioned networking flaws.  
%
%\vspace{-1.0ex}
%\begin{framed}
%\vspace{-1.2ex}
%\noindent
%\textbf{Summary: }{\emph{In general, distributed file systems are much more vulnerable to remote attacks than generic file systems and, hence, much more exploitable. 
%}}
%\vspace{-1ex}
%\end{framed}
%

\begin{table}[t]
	%\vspace{-1ex}
    \footnotesize
    \caption{Quantifying the attack surface of networked \textit{fs}.}
	\vspace{-2ex}
    \label{tab:attacksurface}
    \centering
    \begin{tabular}{|p{32pt}<{\centering}|p{58pt}<{\centering}|p{45pt}<{\centering}|p{40pt}<{\centering}|}
    \hline
    \textbf{FS} & \textbf{User-space APIs} & \textbf{System Calls} & \textbf{RPC/HTTP }  \\
        \hline
	NFS  &  72 & 40 & 108            \\
	OpenAFS  & 35 & 73 &  216        \\
	GlusterFS  & 108 & 64 & 110       \\
    CephFS & 125 & 115 & 32       \\
    %GPFS & 19 & 42 & -       \\
    HDFS & 74 & 20 & 35       \\
        \hline
    \end{tabular}
	\vspace{-4ex}
\end{table}




\subsection{Defense Strategies for Networked FS}
\label{sec:networkedfix}
%\ben{ Reviewer D: ``In 5.6, you may also wish to consider whether an approach to network packet verification such as Chi et al.'s "A system to verify network behavior of known cryptographic clients" from NDSS '17 might be useful to address these issues with network file systems."} 
%Similar to mobile \textit{fs} vulnerabilities, 
The defense strategies used in generic \textit{fs} can also be applied to fix (34.1\%) 
networked \textit{fs} vulnerabilities. 
This is because most networked file systems are built upon the generic \textit{fs} 
(see $\S$~\ref{sec:correlation}).  
%We examine 59 patches that fix the vulnerabilities in distributed \textit{fs} such as NFS, 
%Ceph, and GlusterFS, explore the patterns in them. 
Also, there are unique defense strategies (65.9\%) to networked \textit{fs} as shown in Table~\ref{tab:distfixes}. 
We find that enforcing authentication and access
control is still a simple yet effective way to avoid privilege escalation. 
Beyond this, we identify the following opportunities for enhancing the networked \textit{fs}. 
	
\noindent
\textbf{\texttt{D05:} Network packet verification.} 
According to our study, %on the patches committed to fix those networked \textit{fs} vulnerabilities, 
verifying the network
packets, especially those via the HTTP or RPC protocols, can significantly reduce the risk
of network attacks in networked \textit{fs}.
The semantic specifications from upper-level service protocols defined by network \textit{fs} 
will facilitate such network packet verification. Similar network verification techniques
have been developed in software-defined networking domain~\cite{plankton:nsdi2020, networkv:popl2016}
and packet level authentication~\cite{p4v:sigcomm2018}, however, few of them focused on the 
semantic-aware verification of storage traffic from networked \textit{fs}. 



%\noindent
%\textbf{\texttt{D06:} Verify networked \textit{fs} implementation with VFS specification.} 
%We find that following the generic VFS specification to 
%interact with local \textit{fs} is also critical to ensure the networked \textit{fs} security (see $\S$~\ref{sec:correlation}). 
%And a majority of networked file systems support VFS, however, 
%they may not follow the specifications in their implementations, which causes correlation vulnerabilities when they interact with local \textit{fs}.
%As prior research has developed many system verification~\cite{nelson:sosp2017, gu-osdi16, 
%amani-asplos16,sigurbjarnarson-osdi16,bornholt-asplos16,chen-sosp15,chen-sosp17}, 
%model checking~\cite{yang-osdi04, samc:osdi14, tom:sosp2015}, and bug finding 
%tools~\cite{yang-osdi06, ma:fast2013, min-sosp15} to 
%pinpoint the bugs in \textit{fs}, few studies work on the 
%intersection of networked \textit{fs} and local \textit{fs}. We wish our study would 
%motivate the relevant research and drive the development of these verification tools. 
%
\noindent
\textbf{\texttt{D06:} Fault isolation for networked \textit{fs} instances.} 
As discussed in $\S$~\ref{sec:correlation}, a \textit{fs} instance (e.g., a data volume manager) has 
correlations with many system components such as local \textit{fs} and OS kernel. These correlations 
significantly complicate the management of \textit{fs} instances as well as increase the attack surface. 
Providing a fault isolation mechanism for \textit{fs} instances can significantly enhance the 
security of the entire networked system. Systems techniques, such as containers~\cite{container:acsac18, xcontainer:asplos2019}, 
sandbox~\cite{sandbox:ccs2010}, and TEE~\cite{libseal:eurosys18}, have been proposed to enforce the isolation 
between programs. They can be leveraged to enable isolation between networked \textit{fs} instances. 
However, a holistic approach that requires fine-grained function partition and placement for networked \textit{fs} 
is still highly desirable~\cite{correlated:osdi14}. 

\begin{table}[t]
    \footnotesize
        \caption{Defense strategies for networked \textit{fs} vulnerabilities.}
        \vspace{-2ex}
    \label{tab:distfixes}
    \centering
    \begin{tabular}{|m{160pt}<{\raggedleft}|p{40pt}<{\raggedright}|}
    %\begin{tabular}{r|p{40pt}<{\raggedright}}
                \hline
                \textbf{Unique Defense strategies} & \textbf{\% of CVEs}  \\
        \hline
        Enforce strict authentication/permission control & 26.4\% \\
	Verify (HTTP/RPC) network packets  & 23.1 \%\\
        %Enforce strict user authentication & 15.2\% \\
	%Enforce strict access permission control & 11.2\% \\
	    Enforce VFS specifications  & 9.3\% \\    
	Fault isolation between \textit{fs} instances & 7.1\% \\ 
        %\hline
        % Initialize migration and recovery operations function pointers & 8.4\% \\
        %\hline
        %Prevent getting and setting a file's content using extended attributes & 6.8\% \\
        %\hline
        %Prevent any arbitrary file creation by client & 5.1\% \\
        %\hline
        % Make Ceph Auth Tickets to be of dynamic length & 5.1\% \\
        %\hline
        %Use unique meta-lock for every inode in GlusterFS & 1.7\% \\
        %\hline
        %Ensure a cached page is up-to-date before writing & 1.7\% \\
        %\hline
        %Sort group-ids when setting up user to prevent valid group-ids from getting squashed & 1.7\% \\
        %\hline
        %Place authorization checks for authenticated clients & 1.7\% \\
        %\hline
        %Clear change logs when writing back transactions & 1.7\% \\
        %\hline
        %Others &  23.2\% \\
        \hline
	    (Total) & 65.9\% \\
	    \hline
        %\textbf{Total} & \multicolumn{3}{r}{157}\\
       % \hline
    \end{tabular}
        \vspace{-5ex}
\end{table}

\noindent
\fcolorbox{black}{Gray}{\parbox[c]{8.1cm}{
\textbf{Summary:}\emph{
%34.1\% of networked \textit{fs} vulnerabilities can be addressed with the defense strategies 
%used in generic \textit{fs}. %Specific defense strategies for networked \textit{fs} are still required, 
The most common and effective defense strategies for networked \textit{fs} include user authentication and 
access permission control, and network packet verification. 
%To avoid deep vulnerabilities, 
%special verification tools are needed, such as networked \textit{fs} verification with 
%VFS specification, and fault isolation for \textit{fs} instances. 
		}
}}


==> feature.tex <==

\noindent
\fcolorbox{black}{Gray}{\parbox[c]{8.1cm}{
\textbf{Summary:}\emph{
	Adversaries usually exploit \textit{fs} features that include crash-consistency model and VFS 
	to facilitate their attacks. To alleviate such attacks, we could refine the specifications on 
	the interface between VFS and underlying \textit{fs}, and enforce the correctness of their implementations. 
	%%As more attacks exploit file system features to conduct their attacks, 
	%and most of these vulnerabilities are related to \textit{fs} semantics. 
	%To alleviate such vulnerabilities, we need to refine the specifications on the 
	%interface between VFS and its fs implementations. 
	%and file operations 
	%should be enforced to follow these specifications. 
	%are not easy to detect, due to 
	%the required semantic information. 
	%To defend against such attacks, file systems should integrate security as 
	%an intrinsic property to enforce essential checks in critical system components.
	}
}}
\vspace{-2ex}

\iffalse


\subsubsection{Exploiting FS Bugs}
\label{sec:fsbugs}
The root causes of \textit{fs} vulnerabilities can overlap with the causes of \textit{fs} bugs. 
%as reported in~\cite{lu-fast13}. 
However, %thanks to the existing OS protection and exception handling mechanisms. 
not every bug will 
result in a vulnerability that can be exploited by adversaries. 
To understand how \textit{fs} bugs will lead to serious security vulnerabilities, we re-examine
the bug patches collected in~\cite{fsbug-dataset}. Specifically, we study 1,311 bug patches
related to the causes of \textit{fs} vulnerabilities, and manually check whether
the reported \textit{fs} bug and its fix have the similar pattern as reported in our studied CVEs.

\noindent
\textbf{\texttt{F14:} Not all \textit{fs} bugs are exploited by
adversaries. However, up to 25\% of them can be exploited along with the evolution of \textit{fs} development.} 
%Specifically, we find that 12.5\%--21.2\% of \textit{fs} bugs can be exploited by adversaries on average, 
We demonstrate their distribution in Figure~\ref{fig:kernelbug}.
Note that not all the reported \textit{fs} bugs in the Linux kernel have been submitted to NVD for confirmation.
For these \textit{fs} bugs, their attack vectors are almost the same as discussed in $\S$~\ref{sec:cause}.
Sanity checking and concurrency bugs can be more easily exploited by adversaries (see
Figure~\ref{fig:kernelbug}).
Such a study reflects that the patches committed along the \textit{fs} evolution~\cite{lu-fast13} (i.e., bug fix,
performance optimization, new features, and code maintenance) do introduce security
vulnerabilities with a high possibility.

%\noindent
%\fcolorbox{black}{Gray}{\parbox[c]{8.1cm}{
%\textbf{Finding:}\emph{
%        Not all \textit{fs} bugs will lead to security vulnerabilities that can be exploited by
%        adversaries. However, up to 25\% of them will do along with the \textit{fs} evolution,
%        and sanity checking and concurrency bugs are more easily exploited by adversaries to
%        initiate attacks.
%        }
%}}
%




\subsection{Defense Strategies for Generic FS}
\label{subsec:genericfix}
%\ben{Reviewer D: ``One fairly straightforward conclusion I drew from the paper (and [11]) is that, if at all possible, individual file systems should not be checking permissions at all --- just do it once, correctly in the VFS. One interesting direction for the paper would be to assess whether there are good reasons not to hoist all permission checks into the VFS."}
To understand the defense strategies against generic \textit{fs} vulnerabilities, 
we also study the fixing patches associated 
with each CVE covered in this paper. Although the fix could be ad-hoc for each
individual vulnerability, we summarize the common strategies in Table~\ref{tab:linux-fix}. 
To defend against \textit{sanity checking} vulnerabilities, applying validation checks  
%such as those for segment count and block group flags, 
helps \textit{fs} defend against attacks through mounting maliciously corrupted \textit{fs} images.
%\ben{Reviewer D: ``The discussion of TOCTTOU (p7) is strange, in that most of the TOCTTOU literature describes these as inherent race conditions in an API, not a standard solution. Fixing TOCTTOU vulnerabilities is often non-trivial (for example, see Tsafrir et al.'s FAST '08 best paper), so it is confusing to have this posited as a best practice."}  
As for \textit{concurrency} vulnerabilities, a quick and effective fix is to ensure the 
atomicity of the time-of-check to time-of-use (ToCToU) operations, as they have been widely used 
in \textit{fs} implementations. 
To defend against attacks that exploit \textit{memory errors}, a common 
defense strategy is to initialize allocated data structures (e.g., use-after-free). 
%especially in the fault handlers. 
For the \textit{permission}-related vulnerabilities, as discussed in $\S$~\ref{sec:cause}, 
dedicated vulnerability-detection tools can be developed following specific permission check 
models. 
%enforcing adequate permission checks before allowing users to operate on 
%sensitive data structures like ACLs, has also been an effective strategy. 
%that should be widely adopted for \textit{fs} security. 
Beyond these strategies, we highlight two main techniques to enhance  
\textit{fs} security. %based on our findings.  


\noindent
\textbf{\texttt{D01:}\footnote{We use `D' to represent the defense strategy in this paper.} Verify \textit{fs} implementations with semantics specified in VFS.}  
VFS provides a uniform abstraction level for upper-level programs to interact with 
real \textit{fs} implementations. It offers semantics (e.g., POSIX) for accessing \textit{fs}. 
However, the real \textit{fs} implementation may not exactly satisfy the semantics, due to 
the unclear specifications and software bugs. %This causes a significant number of \textit{fs} vulnerabilities. 
Given that VFS specifications have been defined, they can be refined to 
verify \textit{fs} implementations. 
Prior \textit{fs} verification studies~\cite{nelson:sosp2017, sigurbjarnarson-osdi16} mostly worked on 
crash safety. Our findings reveal that more efforts are required to achieve the end-to-end verification 
of each semantic mapping from the high-level VFS specification to the low-level \textit{fs}
implementation. 

\noindent 
\textbf{\texttt{D02:} Integrity check for \textit{fs} images.}
%\ben{Reviewer B: ``as volumes have become enormous, people have spent decades working on ways to avoid having to do things like the equivalent of a full fsck, which can take a daunting length of time. How do we split the difference and validate the parts that can be used to exploit vulnerabilities and not validate the others (assuming there are any others)?"}
As discussed in $\S$~\ref{subsec:fsfeature}, adversaries can exploit the crash-safety model enforced in modern \textit{fs} to 
initiate their attacks. 
As \textit{fs} provides data durability, the transient errors or modifications to the in-memory data structures would be persisted into the disk (\textit{fs} image), 
causing long-term threats to the host system. Moreover, many attackers can leverage crafted \textit{fs} images to compromise \textit{fs} 
or the entire OS. 
The illegal crafted \textit{fs} image could contain incorrect attributes, invalid link, and illegal data. To defend against such attacks, we need to enforce 
integrity checks before mounting \textit{fs} images. Recent studies have started to develop fuzz testing tools along this direction, such as Janus~\cite{Xu-sp19} and Hydra~\cite{kim:sosp2019}. We believe new tools can be developed with a focus on testing the integrity checks to identify \textit{fs} vulnerabilities.  

%Given crafted \texttt{fs} image security importance, we should have a integrity check before mounting the new image or give legal \texttt{fs} image a certificate authority (CA) so that image only satisfied with integrity check and having CA can be mounted.  Besides, future defense strategies should give the trustable user a warning that the image may be corrupted like android app installation.


%\noindent
%\textbf{\texttt{D03:} Enforce hardware isolation between file blocks.}  
%The increasing complexity of block management in file systems introduces a 
%significant number of vulnerabilities (see $\S$~\ref{sec:dimension2}). 
%As the file blocks and their attributes are stored in the system-wide shared 
%hardware storage device, the compromise of a file (e.g., permission bypass, privilege 
%escalation) produces threats to the collocated files. 
%%Although storage software has implemented access controls and security isolation, 
%Enforcing hardware isolation between file 
%blocks at the device level would enable the access protection fundamentally. This defense 
%is becoming feasible today along with the development of software-defined storage that allows 
%developers to offload and customize functions in storage devices~\cite{devfs-fast2018, lightnvm-fast2017}. 
%
%\noindent
%\textbf{\texttt{D03:} Persistent storage.}  
%\vspace{20ex}
%




%\begin{comment}
%\begin{table}[t]
%    \footnotesize
%        \caption{Fixing strategies for \textit{fs} vulnerabilities.}
%        \vspace{-1ex}
%    \label{tab:fixes}
%    \centering
%    \begin{tabular}{m{175pt}<{\raggedright}|p{40pt}<{\raggedright}}
%                \hline
%                \textbf{Fixing strategies} & \textbf{\% of CVEs}  \\
%        \hline
%        Validate file system image before mounting    & 23.4 \\
%        \hline
%        Fix memory errors on fault-handling paths   & 11.7 \\
%        \hline
%         Check user privileges for ACL modifications, inode encryption policies, etc.  &  11.7 \\
%        \hline
%         Fix file permission checks for ioctl operations on files & 8.8 \\
%        \hline
%        Prevent use of uninitialized or unallocated objects & 8.0\\
%        \hline
%         Check for integer overflows in file sizes and offsets & 7.3 \\
%        \hline
%        Validate of data/pointers copied from user-space & 5.8 \\
%        \hline
%        Make TOCTOU racing operations atomic & 3.7\\
%        \hline
%        Others &  19.6\\
%        \hline
%    \end{tabular}
%    %    \vspace{-3ex}
%\end{table}
%\end{comment}


\noindent
\fcolorbox{black}{Gray}{\parbox[c]{8.1cm}{
	\textbf{Summary: }\emph{
	Common defense strategies can be adopted to enhance \textit{fs} security. They include  
validating \textit{fs} images before mounting, initializing in-memory data 
structures before using them, and \textit{fs} verification with VFS semantics. 
%and enforcing user privileges are the most common and effective fixing strategies.
	}
}}



\fi

==> mobilefs.tex <==
\section{Mobile FS Vulnerability}
\label{sec:mobilefs}
%\ben{Highlight more differences between mobile and general}
%In $\S$~\ref{sec:genericfs}, 
%We conduct the study of generic \textit{fs} vulnerabilities in $\S$~\ref{sec:genericfs}, 
We believe our findings in $\S$~\ref{sec:genericfs} also apply to special \textit{fs}  
running on mobile and distributed platforms. 
According to their higher scores of severity, impact, and 
exploitability (Figure~\ref{fig:dist-mobile-gen}), 
vulnerabilities in mobile and networked \textit{fs} 
are more severe. 
%For those file systems, we are more interested in understanding their unique  
%properties.   

%Mobile devices have become prevalent today, which store substantial personal and sensitive user data. 
%Unfortunately, they have also attracted numerous attacks and suffered from severe security issues~\cite{xu-csur16}. 
To understand those \textit{fs} vulnerabilities, we first present 
our study on mobile \textit{fs} with a focus on their unique properties related to mobiles.  
We focus on the most popular mobile OS such as Android and iOS.
Android is an open-source mobile OS running atop the Linux kernel. 
%Many of its \textit{fs} are derived from Linux generic \textit{fs}. 
As the majority of mobile storage mediums are flash based, we study  
the flash-friendly \textit{fs}, such as F2FS~\cite{lee-fast15}. 
We also study the kernel \textit{fs} (e.g., proc, Ext4, sysfs), which are widely 
used in Android. For iOS, we mainly examine three typical \textit{fs}:   
HFS, HFS+, and APFS. 

\begin{figure}[t]
	\centering
		\vspace{-1.5ex}
	%\begin{minipage}[c]{\linewidth}
		\includegraphics[width=0.95\linewidth]{Figures/allscore.pdf}
		\vspace{-3ex}
	%\end{minipage}
	%\vspace{-1ex}
%	\caption{Comparison of generic, mobile, and networked \textit{fs} vulnerabilities.}
		\caption{Comparison of generic, mobile, and networked \textit{fs} vulnerabilities on different computing platforms.}
	\label{fig:dist-mobile-gen}
	\vspace{-2ex}
\end{figure}



\begin{figure}[t]
        \centering
        \begin{minipage}[c]{\linewidth}
                \includegraphics[width=0.95\linewidth]{Figures/MobileFSAttackModel-new.pdf}
                %\vspace{-4ex}
        \end{minipage}
        %\vspace{-2ex}
        \caption{Attack models in mobile \textit{fs}.}
        \label{fig:mobileattack}
        \vspace{-3ex}
\end{figure}

\subsection{Common Attacks in Mobile FS}
\label{subsec:mobileoverview}

We summarize the attack models in mobile \textit{fs} in Figure~\ref{fig:mobileattack}. 
We identify that a large portion of data leakages are caused by 
the authentication issues in the category of sanity checking, 
including the encryption/decryption key management, cryptographic issues, and volume management. 
Unlike generic \textit{fs} (see Figure~\ref{fig:genericattack}), 
mobile \textit{fs} suffers from more physical attacks (see $\S$~\ref{sec:physical}), due to the 
unique property of mobile devices. 
%Specifically, adversaries usually exploit the vulnerabilities 
%with the adapter and Android Bridge Debugging (ADB) to cause data leakage or privilege escalation.


\noindent
%\textbf{\texttt{F15:} Data leakage is the major consequence of mobile \textit{fs} vulnerabilities.} 
\jinghan{This is wrong. Privilege Escalation is the major attack in mobile fs. DoS is decreasing; Data leakage is increasing. I will help fix it.}
\textbf{\texttt{F15:} DoS is also the major attack in mobile \textit{fs}.} 
%\ben{Reviewer A thinks DoS is more impactful} 
We summarize the distribution of attacks in mobile \textit{fs} in Table~\ref{tab:mobifs-summary}.  
%over 50\% of vulnerabilities in iOS \textit{fs} can be initiated 
%through physical means, 
As we can see, 56\% of \textit{fs} vulnerabilities are related to DoS attack on average. 
Specifically, 83\% of \textit{fs} vulnerabilities in F2FS resulted in DoS attack, 
and nearly 40\% of vulnerabilities in APFS lead to DoS attack. 
%or data leakage,  %whereas 83\% of vulnerabilities in F2FS cause DoS.
We also observe that averagely 17\% of \textit{fs} vulnerabilities caused data leakage, 
and 24\% of them lead to privilege escalation. 
%and 10\% of \textit{fs} vulnerabilities in HFS/HFS+ involve access permission 
%bypass. %Interestingly, 
Interestingly, no reported cases suffer from the attacks of permission bypass in Android. 
%\ben{unclear why data leakage can still happen despite the current encryption support on mobile}

Following the categories of attack vectors discussed in Table~\ref{tab:genericfs}, 
we show their distribution in mobile \textit{fs} vulnerabilities in 
Figure~\ref{fig:mobile-causes}. \textit{Sanity checking}  
constitutes nearly 60\% of the vulnerabilities in HFS/HFS+, APFS (used in iOS), and 
F2FS (used in Android); and memory errors are a main attack vector of nearly 60\% of 
all vulnerabilities in eCryptfs and kernel \textit{fs}. %such as Ext4 and debugfs.
%We present our characteristics study of mobile \textit{fs} in details as follows. 



\begin{comment}
\begin{figure}[t]
	\centering
	%\vspace{-1ex}
	\begin{minipage}[c]{\linewidth}
		\includegraphics[width=0.99\linewidth]{Figures/mobile_cause.pdf}
	%	\vspace{-4ex}
		\label{fig:kernelrel}
	\end{minipage}
	\vspace{-4ex}
	\caption{Attack vectors in mobile \textit{fs}.}
	\label{fig:mobile-causes}
	\vspace{-5ex}
\end{figure}

\end{comment}

%\subsection{Attack Models in Mobile File Systems}
%\label{subsec:mobileattack}
%\ben{would be improved with an example} To understand the attack procedures in mobile \textit{fs}, 


%\subsection{Mobile Data Privacy}
%\label{sec:mobileprivacy}
%With the growing number of mobile applications and large device capacity, substantical sensitive 
%and critical files are stored in the mobile devices. 
\noindent
\textbf{\texttt{F16:} Data privacy is still the top concern in mobile \textit{fs}, 
although encrypted \textit{fs} has been widely used.} 
To protect data privacy, iOS provides a secure encryption 
mechanism for user files~\cite{apfs-cryption}. 
%They could choose either metadata or data encryption for their critical files. 
APFS leverages hardware to accelerate data encryption and decryption. 
F2FS does not support \textit{fs}-level encryption, but it utilizes a cryptographic stacked 
\textit{fs} (eCryptFS) to guarantee data privacy protection. 
%Through our \textit{fs} vulnerability study, 
We find that data leakage is still a severe 
security issue on mobiles 
(e.g., \texttt{CVE-2017-7149, CVE-2017-13786}), %CVE-2016-1919, CVE-2014-9922}), 
although data encryption is available to protect user data. 
%For example, 
%%an eCryptFS key generation vulnerability (\texttt{CVE-2016-1919}), 
%%may cause critical data leakage. %The algorithm shown in the Figure~\ref{fig:CVE-2016-1919} 
%%Specifically, 
%eCryptFS uses an algorithm to generate a 32-byte AES key that combines 
%the user password and 32-byte TIMA (TrustZone-based Integrity Measurement) key.
%%uses a 32 bytes which combining user password and a random 32 bytes. 
%The vulnerability (\texttt{CVE-2016-1919}) occurs because 
%\textit{Base64.getEncoder} expends the input with a ratio of 4:3. This means that only 24 bytes 
%determine the final eCryptFS key %Weak key which less than 8 bytes would be totally ignored. 
%and adversaries can easily crack the key with a brute-force search. 
%Furthermore, 
Mobile \textit{fs} vulnerabilities that cause privacy breaches are 
prevalent in both iOS and Android. As shown in Table~\ref{tab:mobifs-summary}, 
53\% of vulnerabilities in HFS/HFS+ and all the vulnerabilities in APFS (used in iOS)  
caused privacy issues. We observe similar trend in F2FS and eCryptFS used in Android. 
\jinghan{Replace CVE-2017-7149 with some iOS bugs.}
%while 35\% of vulnerabilities in F2FS and 75\% of vulnerabilities in 
%eCryptFS (used in Android) can cause privacy breaches. 
According to our study, adversaries often exploit the encryption/decryption key management to initiate the attacks 
for data leakage (e.g., \texttt{CVE-2016-1919}). 

%\subsection{Mobile Trusted Execution Environment}
%\label{sec:tee}
%In addition to implementation errors in eCryptFS to leak user data from Samsung KNOX TrustZone mentioned in \S~\ref{sec:mobileprivacy}, a local user/malicious application can also exploit the semantic errors in eCryptFS to cause leakage of sensitive kernel data. For instance, a vulnerability reported in eCryptFS, \texttt{CVE-2009-0787}, lead to leakage of kernel data as a result of out-of-bounds read triggered from allocation of incorrect size of eCryptFS file header. 
%\ben{Reviewer D: ``The discussion of TEEs struck me as particularly misleading. The issue amounts to some very sensitive infrastructure being outside of the TEE. So it is true in a facile sense that thunking down a TEE and not using it is, in fact "not sufficient". It would be more accurate to say that TEEs are under-utilized, but the text implies a fundamental drawback that is not supported by the evidence."}

\noindent
\textbf{\texttt{F17:} Mobile TEE is not sufficient to protect (encrypted) mobile \textit{fs}.} 
As trusted execution environment (TEE) has become a standard on mobile devices, 
mobile \textit{fs} can leverage its enabled isolated environment to protect critical 
data from potential vulnerabilities and attacks. However, a drop-in deployment of TEE is insufficient to 
protect \textit{fs}, due to the improper interactions with TEE. %The \textit{fs} vulnerabilities is still exploited, even with the assistance of TEE.
We show an example attack procedure as follows. 
%For example, on a TrustZone-enabled ARM platform, 
When a system crash happens in the non-secure domain of a TrustZone-enabled ARM platform,   
it will trigger an interrupt to switch the system context to the secure domain. Therefore, 
we can access CPU, memory, and register states. As shown in \texttt{CVE-2009-2908}, 
an armored malware can prevent the non-secure domain to issue the interrupt, and then initiate a 
Man-in-the-Middle (MITM) attack to obtain the execution information. Such attack even poses threats 
to encrypted \textit{fs} like eCryptFS, in which it relies on a Volume Daemon (\texttt{vold}) to 
manage mobile storage devices. As \texttt{vold} does not reside in TrustZone, it could be 
exploited to opportunistically leak the encryption keys of eCryptFS from \texttt{vold}'s memory. 
Therefore, malicious users can decrypt user data in TrustZone. %~\cite{kanonov2016secure}.
%\jian{need more insights}
%\ben{Qualcomm appears to have created a "Secure FS" inside the TEE. They claim this is secure though it has some attached CVE's: CVE-2016-10242, CVE-2015-9069, CVE-2014-9952, CVE-2014-9944. Unfortunately, no details are disclosed regarind the nature/casuses of the vulnerabilities. An interesting SoK paper for SSP 2020 (https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=9152801) provides a study on TEE vulnerabilities from 2013-18. Many of the bugs plaguing TEE are similar to what we see in FS (sanity checks missing, etc), but they provide some interesting insights. For one, the number and type of bugs is higher than the corresponding time period for Linux/other OS'es which they say indicates poor development practices. TEE vulnerabilities can be used to take control over the TEE kernel or the Linux kernel using existing CVE exploits. All of this would indicate that relying on the TEE to provide the solutions to our problems naive. Particularly interesting to FS implementations are: Issues in the TA itself that ensures separation of apps, TOCTOU issues, cache vulnerabilities, bugs in peripherals, and bugs in the security mechanism (such as encryption). The remaining bugs could influence the FS in that they can contribute to privilege escalation affecting the FS but would not make the FS itself a vulnerable components within the TEE.}
\noindent
\fcolorbox{black}{Gray}{\parbox[c]{8.1cm}{
\textbf{Summary:}\emph{
DoS and data leakage are the major attacks in mobile \textit{fs}. 
Similar to generic \textit{fs}, sanity check and memory errors are the top 
attack vectors. 
%Although trusted execution environment like TrustZone and encryption file systems like eCryptFS are both 
%enabled, data leakage can still happen in mobile \textit{fs}. 
        }
}}
\vspace{-2ex}


\subsection{Physical vs. Remote Attack}
\label{sec:physical}
As mobile devices are portable, it is interesting to understand what common attack 
approaches (physical vs. remote attack) are used by adversaries, which would provide guidance 
for mobile vendors to enhance their protection strategies. 

\noindent
\textbf{\texttt{F18:} Most mobile \textit{fs} vulnerabilities are exploited by physical attacks.}
%According to our study, 
We find that 
up to 83\% of the mobile \textit{fs} vulnerabilities are exploited by physical attacks (see Table~\ref{tab:mobifs-summary}), and 
75\% of such attacks cause privacy breaches. For example, a case reported in APFS 
(e.g., \texttt{CVE-2017-13786}) was exploited to steal user data. 
Specifically, if a mobile device is connected to a malicious 
Thunderbolt adapter, malicious users can access decrypted data via a DMA access control flaw. 
Another example is Android Debug Bridge (ADB) attack, in which adversaries can exploit  
the command-line debugging tool connected with Android devices to steal user data and modify 
mobile applications (e.g., \texttt{CVE-2017-10662, CVE-2014-7951, CVE-2012-5564}).


\noindent
\textbf{\texttt{F19:} Remote attacks are more exploitable than physical attacks in mobile \textit{fs}.} 
%Remote attacks are more exploitable than physical attacks 
This is because remote attacks usually exploit missing/inappropriate sanity checks while mounting \textit{fs} images, 
whereas physical attacks exploit buffer overflow and data races that are much harder to trigger.
%Beyond physical attacks, adversaries also exploit remote attacks 
38\% of the mobile \textit{fs} vulnerabilities were caused by remote attacks. Adversaries can use malicious programs (e.g., 
\texttt{CVE-2015-3721}) or crafted files (e.g., \texttt{CVE-2016-8463}) to trigger the \textit{fs} 
vulnerability, and cause device hang and data leakage.   
%However, we should also pay attention to the remote attacks (41\% of the total vulnerabilities reported in mobile file systems, of which 46\% of them cause privacy breaches). For example, the adversary could use malicious app (\texttt{CVE-2015-3721}) or crafted file (\texttt{CVE-2016-8463}) to trigger the vulnerabilities, which could have to severe consequences, such as device hang and data leakage. Some vulnerabilities in file systems running in presence of Trusted Execution Environments (TEE) can be very exploitable and can be highly dangerous in terms of the impact on the system. One example of such a highly severe vulnerability is \texttt{CVE-2014-9922} (severity score of 9.3, impact score of 10 and exploitability score of 8.6) found in stackable file systems such as eCryptFS, which could be remotely exploited by recursively stacking eCryptFS and/or also stacking OverlayFS on the top of it or vice versa. This happens due to lack of imposition of an explicit limit on the stack depth for a file system and this can lead to data leakage/modification, disruption of service and even privilege escalation in a TEE due to inherent vulnerabilities in stackable file systems.
There are also many attacks that can be launched remotely but require the interactions with local victims. %or direct physical access to an Android device. 
For instance, 23\% of reported mobile \textit{fs} vulnerabilities (e.g., \texttt{CVE-2018-13096}, 
\texttt{CVE-2018-13097}) %\texttt{CVE-2018-13100}, etc.) 
are exploitable with evil-maid attacks or voluntary interaction with victim users. 
Most of such attacks are launched by mounting crafted files that exploit missing checks for 
division-by-zero or NULL pointer dereferences. 
%Note that no authentication is required by an evil-maid attacker to render an Android device. 
%completely unavailable to the owner.


\noindent
\fcolorbox{black}{Gray}{\parbox[c]{8.1cm}{
\textbf{Summary:}\emph{
	Physical attack is more popular than remote attack to exploit mobile \textit{fs} vulnerabilities 
	in both Android and iOS. However, remote attack is highly exploitable and can be 
	as severe as physical attack.
        }
}}
\vspace{-3ex}







\subsection{Defense Strategies for Mobile FS}
\label{sec:mobilefix}
As discussed in $\S$~\ref{subsec:mobileoverview}, many mobile file systems were developed based on the 
generic \textit{fs}. The common defense strategies discussed in $\S$~\ref{subsec:genericfix} 
can be applied to fix the (43.7\%) mobile \textit{fs} vulnerabilities. Meanwhile, we identify the 
unique defense strategies for mobile \textit{fs} vulnerabilities, as shown in Table~\ref{tab:mobfixes}.  


\noindent
\textbf{\texttt{D03:} Enhance secure channels between mobiles and external physical devices.} 
To defend against physical attacks, we need to continue developing secure channels between mobile devices and 
external devices such as Thunderbolt adapters and USB ports. 
%Specifically, 
%we find that adding authentication mechanisms to secure ADB channels between ADB host  
%and client can avoid ADB-related attacks. %and mitigate 25\% of mobile \textit{fs} vulnerabilities. 
%\cite{hwang2015bittersweet}. 
As discussed in $\S$~\ref{sec:physical}, nearly 23\% of vulnerabilities in Android can be 
exploited by evil-maid attacks. These attacks can be prevented by explicitly authorizing the 
mounting of external devices. 
%Moreover, we find that enhancing the security of 
%USB-debugging mode (enabled by default on Android devices) or directly disabling it can avoid 
%physical ADB attacks. 

\noindent
\textbf{\texttt{D04:} Enforce secure communication between TEE and \textit{fs}.} 
We still cannot solely rely on TEE or encryption \textit{fs} or even both to 
ensure the security of mobile \textit{fs}. Particularly, we have to ensure the secure interactions between 
TEE and \textit{fs}, such as preventing the direct access to the memory used by Volume Daemon or storage 
management process from TrustZone. We have to carefully refine the interface between the TEE and 
file systems, which can be improved with the development of both TEE and file system side~\cite{sok-oakland2020, android-ecosystem, android:csur}. 


\noindent
\fcolorbox{black}{Gray}{\parbox[c]{8.1cm}{
\textbf{Summary:}\emph{
	The defense strategies for generic fs can definitely be applied to mobile fs, 
	we find 43.7\% of mobile fs vulnerabilities have been addressed with them. 
	Meanwhile, unique strategies, such as securing ADB channels and interaction with 
	TEE, are also desired. 
        }
}}
	\vspace{-2ex}



==> scores.tex <==
%\section{<Add Section Name>}
%\label{sec:scores}
%
%In this section we study the vulnerbility metrics for file systems in linux kernel and use them to explore the relation of the vulnerabilities found in file systems in Linux kernel with other kernel components. Also, we study the security bugs in the aforementioned file systems that have gone unreported as CVEs.
%
%\subsection{Common Vulnerability Metrics}
%The Information Technology Laboratory (ITL) provides a National Vulnerability Database that contains all the reported CVEs and defines vulnerability metrics that constitute three scores denoting severity, impact and exploitability. All scores are ranged between 1 to 10, and in this paper, 0 to 3.9 score  denotes low, 4.0 to 6.9 score range denotes medium and 7.0 to 10.0 score range denotes high levels of severity, impact or exploitability. These metrics quantitatively insights into vulnerabilties and exploits, and help compare different file systems and their vulnerabilities. 

We studied how severe, impactful and exploitable the vulnerabilities in file systems in Linux kernel are. We found that Linux kernel file systems studied above have, on an average, medium level of severity (low: 18.7\%, medium: 65.5\%, high: 15.8\%), medium level of impact (low: 36.5\%, medium: 48.2\%, high: 15.3\%) and low level of exploitability (low: 84.7\%, medium: 1.3\%, high: 14.0\%). 

Figure~\ref{fig:impactpercent} shows percentage of impact levels of vulnerabilities in every Linux kernel file system we studied due to different causes. 


%\begin{figure*}[h]
%	\centering
%	\begin{minipage}[c]{.3\linewidth}
%    	\includegraphics[width=\linewidth]{Figures/basescore.pdf}
    	%\subcaption{Consequences}
%    	\vspace{-1ex}
%    	\label{fig:basescore}
%	\end{minipage}
%	\begin{minipage}[c]{.3\linewidth}
%		\includegraphics[width=\linewidth]{Figures/impactscore.pdf}
		%\subcaption{Consequences}
%		\vspace{-1ex}
%		\label{fig:impactscore}
%	\end{minipage}
	%\hspace{-3ex}
%	\begin{minipage}[c]{.3\linewidth}
%		\includegraphics[width=\linewidth]{Figures/exploitabilityscore.pdf}
		%\subcaption{}
%		\vspace{-1ex}
%		\label{fig:exploitability}
%	\end{minipage}
%	\vspace{-3ex}
%	\caption{Breakdown of different vulnerability metrics for each cause of CVEs}
%\end{figure*}

%\begin{figure*}[t]
%	\centering
%	\begin{minipage}[c]{\linewidth}
%		\includegraphics[width=\linewidth]{Figures/impact_percent.pdf}
%		\vspace{-3ex}
%		\label{fig:kernelrel}
%	\end{minipage}
%	\caption{Impact levels of CVEs in each file system due to different causes}
%	\label{fig:impactpercent}
%	%\vspace{-3ex}
%\end{figure*}

%\subsection{Unreported Security Vulnerabilities}
%Linux Kernel Security Team is not required to 

%\begin{figure*}[t]
%	\centering
%	\begin{minipage}[c]{\linewidth}
%		\includegraphics[width=\linewidth]{Figures/security_bugs_bar_cluster.pdf}
%		\vspace{-3ex}
%		\label{fig:kernelrel}
%	\end{minipage}
%	\caption{Percentage of bugs that can lead to security vulnerabilities}
%	\vspace{-3ex}
%\end{figure*}


%\subsection{Relation with Other Kernel Components}
%Several kernel components including the virtual memory manager, file systems and device drivers have been studied in the past extensively~\cite{Huang-atc16, lu-fast13, kadav2012understanding}. However, security vulnerabilities in those components are not well studied. We looked at the vulnerabilities in core components of the Linux kernel to compare their vulnerability metrics (severity, impact and exploitability) with the file systems as shown in Figure~\ref{fig:kernel-scores}. Vulnerabilities in file systems have higher severity, impact and vulnerability scores on an average compared to other components, excepting the network component which has slightly higher exploitability score since most of its vulnerabilities are exploitable remotely (and hence higher severity). This shows that studying file systems closely all the more important, not just because they provide interface to storage for virtual memory manager, device drivers, applications in userspace, etc., but also because of the inherent nature of the vulnerabilities in terms on their impact and exploitability. 
%
%\begin{figure}[t]
%	\centering
%	\begin{minipage}[c]{\linewidth}
%		\includegraphics[width=\linewidth]{Figures/kernel_components_scores.pdf}
%		\vspace{-5ex}
%	\end{minipage}
%	\caption{Vulnerability Metrics of Linux kernel components}
%	\label{fig:kernel-scores}
%	\vspace{-3ex}
%\end{figure}

